Guidance and Control Networks with Periodic Activation Functions

Inspired by the versatility of sinusoidal representation networks (SIRENs), we present a modified Guidance & Control Networks (G&CNETs) variant using periodic activation functions in the hidden layers. We demonstrate that the resulting G&CNETs train faster and achieve a lower overall training error on three different control scenarios on which G&CNETs have been tested previously. A preliminary analysis is presented in an attempt to explain the superior performance of the SIREN architecture for the particular types of tasks that G&CNETs excel on.

==> gcnet_architectures.tex <==
\begin{figure}[tb]
\centering
\def\layersep{2cm}
\def\nodesep{0.3cm}

\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep, scale=0.7]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=5pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=gray!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{output neuron2}=[neuron, fill=green!50];

    \tikzstyle{hidden neuron softplus}=[neuron, fill=blue!50];

    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \node[input neuron, pin=left:$x$] (I-1) at (0,-\nodesep*1*1.63) {};
    \node[input neuron, pin=left:$y$] (I-2) at (0,-\nodesep*2*1.63) {};
    \node[input neuron, pin=left:$z$] (I-3) at (0,-\nodesep*3*1.63) {};
    \node[input neuron, pin=left:$v_x$] (I-4) at (0,-\nodesep*4*1.63) {};
    \node[input neuron, pin=left:$v_y$] (I-5) at (0,-\nodesep*5*1.63) {};
    \node[input neuron, pin=left:$v_z$] (I-6) at (0,-\nodesep*6*1.63) {};
    % \node[input neuron, pin=left:$m$] (I-7) at (0,-\nodesep*7*1.63) {};

    % \node[] (L0) at (0,-\nodesep*7*1.63-4.6*\nodesep) {$L^{(0)}$};


    % Draw the hidden layer 1 nodes
    \foreach \name / \y in {1,...,14}
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H1-\name) at (\layersep,-\nodesep*\y) {};
    % \node[] (L1) at (\layersep,-\nodesep*15-1*\nodesep) {$L^{(1)}$};

            
    % Draw the hidden layer 2 nodes
    \foreach \name / \y in {1,...,14}
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H2-\name) at (2*\layersep,-\nodesep*\y) {};
    % \node[] (L2) at (2*\layersep,-\nodesep*15-1*\nodesep) {$L^{(2)}$};
            
    % Draw the hidden layer 3 nodes
    \foreach \name / \y in {1,...,14}
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H3-\name) at (2.5*\layersep,-\nodesep*\y) {};
    % \node[] (Ll) at (2.5*\layersep,-\nodesep*15-1*\nodesep) {$L^{(l)}$};

    % Draw the output neurons
    % \node[output neuron2, pin={[pin edge={->}]right:$i_x$}, right of=H3-3] (O-1) at (2.3*\layersep,-1.8)  {};

    \node[output neuron2, pin={[pin edge={->}]right:$i_x$}, right of=H3-3] (O-1) at (2.3*\layersep,-1.2)  {};
    \node[output neuron2, pin={[pin edge={->}]right:$i_y$}, right of=H3-3] (O-2) at (2.3*\layersep,-1.8)  {};
    \node[output neuron2, pin={[pin edge={->}]right:$i_z$}, right of=H3-3] (O-3) at (2.3*\layersep,-2.4)  {};

    
    % \node[below of=O-2] (Ll1) at (3.8*\layersep,-6.6*\nodesep) {$L^{(l+1)}$};


    % Connect every node in the input layer with every node in the
    % hidden layer2.
    \foreach \source in {1,...,6}
        \foreach \dest in {1,...,14}
            \path (I-\source) edge (H1-\dest);
            
    % Connect every node in the hidden layer1 with the hidden layer 2
    \foreach \source in {1,...,14}
        \foreach \dest in {1,...,14}
            \path (H1-\source) edge (H2-\dest);

    % Draw the dots for the missing layers      
    \path[thick] ([xshift=.1cm] H2-8.east) edge[-,loosely dotted] ([xshift=.1cm] H3-8.east);

    % Connect every node in the hidden layer 3 with the output layer
    \foreach \source in {1,...,14}
        \foreach \dest in {1,...,3}
            \path (H3-\source) edge (O-\dest);

    \pgfmathsetmacro{\scale}{0.2}
    \pgfmathsetmacro{\Ox}{10}
    \pgfmathsetmacro{\Oy}{4}

    % Plot nonlinearities
    \draw[scale=\scale, shift = {(\Ox, \Oy)}] (-3,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox, \Oy)}] (0,-1) -- (0,3) node[above] {softplus};
    \draw[scale=\scale,domain=-3:3,smooth,variable=\x,blue, shift = {(\Ox, \Oy)} ] plot ({\x},{ln(1+exp(\x)});
    
    \draw[scale=\scale, shift = {(\Ox+10, \Oy)}] (-3,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox+10, \Oy)}] (0,-1) -- (0,3) node[above] {};
    \draw[scale=\scale,domain=-3:3,smooth,variable=\x,blue, shift = {(\Ox+10, \Oy)} ] plot ({\x},{ln(1+exp(\x)});
    
    \draw[scale=\scale, shift = {(\Ox+15, \Oy)}] (-1,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox+15, \Oy)}] (0,-1) -- (0,3) node[above] {};
    \draw[scale=\scale,domain=-2:3,smooth,variable=\x,blue, shift = {(\Ox+15, \Oy)} ] plot ({\x},{ln(1+exp(\x)});
    
    \draw[scale=\scale, shift = {(\Ox+30, \Oy-5)}] (-1,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox+30, \Oy-5)}] (0,-1) -- (0,3) node[above] {linear};
    \draw[scale=\scale,domain=-2:3,smooth,variable=\x,green, shift = {(\Ox+30, \Oy-5)} ] plot ({\x},{(\x)});

\end{tikzpicture}
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep, scale=0.7]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=5pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=gray!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{output neuron2}=[neuron, fill=green!50];

    \tikzstyle{hidden neuron softplus}=[neuron, fill=blue!50];

    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \node[input neuron, pin=left:$x$] (I-1) at (0,-\nodesep*1*1.63) {};
    \node[input neuron, pin=left:$y$] (I-2) at (0,-\nodesep*2*1.63) {};
    \node[input neuron, pin=left:$z$] (I-3) at (0,-\nodesep*3*1.63) {};
    \node[input neuron, pin=left:$v_x$] (I-4) at (0,-\nodesep*4*1.63) {};
    \node[input neuron, pin=left:$v_y$] (I-5) at (0,-\nodesep*5*1.63) {};
    \node[input neuron, pin=left:$v_z$] (I-6) at (0,-\nodesep*6*1.63) {};
    \node[input neuron, pin=left:$m$] (I-7) at (0,-\nodesep*7*1.63) {};

    % \node[] (L0) at (0,-\nodesep*7*1.63-4.6*\nodesep) {$L^{(0)}$};


    % Draw the hidden layer 1 nodes
    \foreach \name / \y in {1,...,15}
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H1-\name) at (\layersep,-\nodesep*\y) {};
    % \node[] (L1) at (\layersep,-\nodesep*15-1*\nodesep) {$L^{(1)}$};

            
    % Draw the hidden layer 2 nodes
    \foreach \name / \y in {1,...,15}
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H2-\name) at (2*\layersep,-\nodesep*\y) {};
    % \node[] (L2) at (2*\layersep,-\nodesep*15-1*\nodesep) {$L^{(2)}$};
            
    % Draw the hidden layer 3 nodes
    \foreach \name / \y in {1,...,15}
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H3-\name) at (2.5*\layersep,-\nodesep*\y) {};
    % \node[] (Ll) at (2.5*\layersep,-\nodesep*15-1*\nodesep) {$L^{(l)}$};

    % Draw the output neurons
    \node[output neuron, pin={[pin edge={->}]right:$u$}, right of=H3-3] (O-1) at (2.3*\layersep,-0.2)  {};
    \node[output neuron2, pin={[pin edge={->}]right:$i_x$}, right of=H3-3] (O-2) at (2.3*\layersep,-3)  {};
    \node[output neuron2, pin={[pin edge={->}]right:$i_y$}, right of=H3-3] (O-3) at (2.3*\layersep,-3.4)  {};
    \node[output neuron2, pin={[pin edge={->}]right:$i_z$}, right of=H3-3] (O-4) at (2.3*\layersep,-3.8)  {};
    % \node[below of=O-2] (Ll1) at (3.8*\layersep,-6.6*\nodesep) {$L^{(l+1)}$};


    % Connect every node in the input layer with every node in the
    % hidden layer2.
    \foreach \source in {1,...,7}
        \foreach \dest in {1,...,15}
            \path (I-\source) edge (H1-\dest);
            
    % Connect every node in the hidden layer1 with the hidden layer 2
    \foreach \source in {1,...,15}
        \foreach \dest in {1,...,15}
            \path (H1-\source) edge (H2-\dest);

    % Draw the dots for the missing layers      
    \path[thick] ([xshift=.1cm] H2-8.east) edge[-,loosely dotted] ([xshift=.1cm] H3-8.east);

    % Connect every node in the hidden layer 3 with the output layer
    \foreach \source in {1,...,15}
        \foreach \dest in {1,...,4}
            \path (H3-\source) edge (O-\dest);

    \pgfmathsetmacro{\scale}{0.2}
    \pgfmathsetmacro{\Ox}{10}
    \pgfmathsetmacro{\Oy}{4}

    % Plot nonlinearities
    \draw[scale=\scale, shift = {(\Ox, \Oy)}] (-3,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox, \Oy)}] (0,-1) -- (0,3) node[above] {softplus};
    \draw[scale=\scale,domain=-3:3,smooth,variable=\x,blue, shift = {(\Ox, \Oy)} ] plot ({\x},{ln(1+exp(\x)});
    
    \draw[scale=\scale, shift = {(\Ox+10, \Oy)}] (-3,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox+10, \Oy)}] (0,-1) -- (0,3) node[above] {};
    \draw[scale=\scale,domain=-3:3,smooth,variable=\x,blue, shift = {(\Ox+10, \Oy)} ] plot ({\x},{ln(1+exp(\x)});
    
    \draw[scale=\scale, shift = {(\Ox+15, \Oy)}] (-1,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox+15, \Oy)}] (0,-1) -- (0,3) node[above] {};
    \draw[scale=\scale,domain=-2:3,smooth,variable=\x,blue, shift = {(\Ox+15, \Oy)} ] plot ({\x},{ln(1+exp(\x)});
    
    \draw[scale=\scale, shift = {(\Ox+30, \Oy-2)}] (-1,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox+30, \Oy-2)}] (0,-1) -- (0,3) node[above] {sigmoid};
    \draw[scale=\scale,domain=-2:3,smooth,variable=\x,red, shift = {(\Ox+30, \Oy-2)} ] plot ({\x},{1/(1+exp(-\x * 2))});
    
    \draw[scale=\scale, shift = {(\Ox+30, \Oy-15)}] (-1,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox+30, \Oy-15)}] (0,-1) -- (0,3) node[above] {linear};
    \draw[scale=\scale,domain=-2:3,smooth,variable=\x,green, shift = {(\Ox+30, \Oy-15)} ] plot ({\x},{(\x)});
    
    %\draw[scale=\scale,domain=-3:3,smooth,variable=\x,red, shift = {(\Ox, \Oy)} ] plot ({\x},{tanh(\x)});
\end{tikzpicture}
\caption{G\&CNET architectures: transfer (top) and landing (bottom). Adapted from \cite{izzo2021real}. \label{fig:ffnn}}

\end{figure}

==> gcnet_drone.tex <==
\begin{figure}[tb]
\centering
\def\layersep{2cm}
\def\nodesep{0.3cm}

\begin{tikzpicture}
  \includegraphics[width=0.7\columnwidth]{figures/FBD_Bebop.pdf}
\end{tikzpicture}

\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep, scale=0.7]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=5pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=gray!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{output neuron2}=[neuron, fill=green!50];

    \tikzstyle{hidden neuron softplus}=[neuron, fill=blue!50];

    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \node[input neuron, pin=left:$x$] (I-1) at (0,-\nodesep*1*1.63) {};
    \node[input neuron, pin=left:$y$] (I-2) at (0,-\nodesep*2*1.63) {};
    \node[input neuron, pin=left:$z$] (I-3) at (0,-\nodesep*3*1.63) {};
    \node[input neuron, pin=left:$v_x$] (I-4) at (0,-\nodesep*4*1.63) {};
    \node[input neuron, pin=left:$v_y$] (I-5) at (0,-\nodesep*5*1.63) {};
    \node[input neuron, pin=left:$v_z$] (I-6) at (0,-\nodesep*6*1.63) {};
    \node[input neuron, pin=left:$m$] (I-7) at (0,-\nodesep*7*1.63) {};

    % \node[] (L0) at (0,-\nodesep*7*1.63-4.6*\nodesep) {$L^{(0)}$};


    % Draw the hidden layer 1 nodes
    \foreach \name / \y in {1,...,15}
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H1-\name) at (\layersep,-\nodesep*\y) {};
    % \node[] (L1) at (\layersep,-\nodesep*15-1*\nodesep) {$L^{(1)}$};

            
    % Draw the hidden layer 2 nodes
    \foreach \name / \y in {1,...,15}
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H2-\name) at (2*\layersep,-\nodesep*\y) {};
    % \node[] (L2) at (2*\layersep,-\nodesep*15-1*\nodesep) {$L^{(2)}$};
            
    % Draw the hidden layer 3 nodes
    \foreach \name / \y in {1,...,15}
        \path[yshift=0.5cm]
            node[hidden neuron softplus] (H3-\name) at (2.5*\layersep,-\nodesep*\y) {};
    % \node[] (Ll) at (2.5*\layersep,-\nodesep*15-1*\nodesep) {$L^{(l)}$};

    % Draw the output neurons
    \node[output neuron, pin={[pin edge={->}]right:$u$}, right of=H3-3] (O-1) at (2.3*\layersep,-0.2)  {};
    \node[output neuron2, pin={[pin edge={->}]right:$i_x$}, right of=H3-3] (O-2) at (2.3*\layersep,-3)  {};
    \node[output neuron2, pin={[pin edge={->}]right:$i_y$}, right of=H3-3] (O-3) at (2.3*\layersep,-3.4)  {};
    \node[output neuron2, pin={[pin edge={->}]right:$i_z$}, right of=H3-3] (O-4) at (2.3*\layersep,-3.8)  {};
    % \node[below of=O-2] (Ll1) at (3.8*\layersep,-6.6*\nodesep) {$L^{(l+1)}$};


    % Connect every node in the input layer with every node in the
    % hidden layer2.
    \foreach \source in {1,...,7}
        \foreach \dest in {1,...,15}
            \path (I-\source) edge (H1-\dest);
            
    % Connect every node in the hidden layer1 with the hidden layer 2
    \foreach \source in {1,...,15}
        \foreach \dest in {1,...,15}
            \path (H1-\source) edge (H2-\dest);

    % Draw the dots for the missing layers      
    \path[thick] ([xshift=.1cm] H2-8.east) edge[-,loosely dotted] ([xshift=.1cm] H3-8.east);

    % Connect every node in the hidden layer 3 with the output layer
    \foreach \source in {1,...,15}
        \foreach \dest in {1,...,4}
            \path (H3-\source) edge (O-\dest);

    \pgfmathsetmacro{\scale}{0.2}
    \pgfmathsetmacro{\Ox}{10}
    \pgfmathsetmacro{\Oy}{4}

    % Plot nonlinearities
    \draw[scale=\scale, shift = {(\Ox, \Oy)}] (-3,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox, \Oy)}] (0,-1) -- (0,3) node[above] {softplus};
    \draw[scale=\scale,domain=-3:3,smooth,variable=\x,blue, shift = {(\Ox, \Oy)} ] plot ({\x},{ln(1+exp(\x)});
    
    \draw[scale=\scale, shift = {(\Ox+10, \Oy)}] (-3,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox+10, \Oy)}] (0,-1) -- (0,3) node[above] {};
    \draw[scale=\scale,domain=-3:3,smooth,variable=\x,blue, shift = {(\Ox+10, \Oy)} ] plot ({\x},{ln(1+exp(\x)});
    
    \draw[scale=\scale, shift = {(\Ox+15, \Oy)}] (-1,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox+15, \Oy)}] (0,-1) -- (0,3) node[above] {};
    \draw[scale=\scale,domain=-2:3,smooth,variable=\x,blue, shift = {(\Ox+15, \Oy)} ] plot ({\x},{ln(1+exp(\x)});
    
    \draw[scale=\scale, shift = {(\Ox+30, \Oy-2)}] (-1,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox+30, \Oy-2)}] (0,-1) -- (0,3) node[above] {sigmoid};
    \draw[scale=\scale,domain=-2:3,smooth,variable=\x,red, shift = {(\Ox+30, \Oy-2)} ] plot ({\x},{1/(1+exp(-\x * 2))});
    
    \draw[scale=\scale, shift = {(\Ox+30, \Oy-15)}] (-1,0) -- (3,0) node[right] {};
    \draw[scale=\scale, shift = {(\Ox+30, \Oy-15)}] (0,-1) -- (0,3) node[above] {linear};
    \draw[scale=\scale,domain=-2:3,smooth,variable=\x,green, shift = {(\Ox+30, \Oy-15)} ] plot ({\x},{(\x)});
    
    %\draw[scale=\scale,domain=-3:3,smooth,variable=\x,red, shift = {(\Ox, \Oy)} ] plot ({\x},{tanh(\x)});
\end{tikzpicture}

% \caption{G\&CNET architectures: transfer (top) and landing (bottom). Adapted from \cite{izzo2021real}. \label{fig:ffnn}}

\end{figure}
